Testing Product Distributions: A Closer Look

We study the problems of identity and closeness testing of $n$-dimensional product distributions. Prior works by Canonne, Diakonikolas, Kane and Stewart (COLT 2017) and Daskalakis and Pan (COLT 2017) have established tight sample complexity bounds for non-tolerant testing over a binary alphabet: given two product distributions $P$ and $Q$ over a binary alphabet, distinguish between the cases $P = Q$ and $d_{\mathrm{TV}}(P, Q) > \epsilon$. We build on this prior work to give a more comprehensive map of the complexity of testing of product distributions by investigating tolerant testing with respect to several natural distance measures and over an arbitrary alphabet. Our study gives a fine-grained understanding of how the sample complexity of tolerant testing varies with the distance measures for product distributions. In addition, we also extend one of our upper bounds on product distributions to bounded-degree Bayes nets.

==> MissingLB.tex <==
\section{Missing Proofs from Lower Bounds}
\relFdelP*

\begin{proof}
Let $P=\langle p_1,\dots,p_i,\dots,p_n \rangle$ and $Q=\langle q_1,\dots,q_i,\dots,q_n \rangle$ be the probability values of $P$ and $Q$.
\begin{align*}
\dtv(F_{\delta}(P),F_{\delta}(Q))&=\sum_{x \in \{0,1\}^n} |F_{\delta}(P)(x)-F_{\delta}(Q)(x)|\\ 
&\ge \sum_{i=1}^n |F_{\delta}(P)(e_i)-F_{\delta}(Q)(e_i)| &&\tag{unit vector $e_i$ has $i$-th value 1}\\
&= \sum_{i=1}^n |(1-e^{-\delta p_i})\Pi_{j\neq i} e^{-\delta p_j}-(1-e^{-\delta q_i})\Pi_{j\neq i} e^{-\delta q_j}|\\
&= \sum_{i=1}^n e^{-\delta} |e^{\delta p_i}-e^{\delta q_i}| &&\tag{Since $\Pi_{j} e^{-\delta p_j}=\Pi_{j} e^{-\delta q_j}=e^{-\delta}$}\\
&= e^{-\delta} \sum_{i=1}^n |\delta(p_i-q_i)+\delta^2(p_i^2-q_i^2)/2!+\dots+\delta^j(p_i^j-q_i^j)/j!+\dots|.
\end{align*}
We analyze the expression under modulus under two cases: 1) if $p_i > q_i$, it is more than $\delta(p_i-q_i)$, 2) if $p_i < q_i$, it is more than $\delta(q_i-p_i)$.
\begin{align*}
\dtv(F_{\delta}(P),F_{\delta}(Q))&\ge e^{-\delta}\sum_{i=1}^n |\delta(p_i-q_i)|\\
&=\delta e^{-\delta} \dtv(P,Q).
\end{align*} 
\end{proof}

\chisqFdelta*
\begin{proof}
From \cref{fact-fdeltap}, both $F_{\delta}(P)$ and $F_{\delta}(Q)$ are product distributions, the 
distribution of the $i$-th component being $F_{\delta}(P_i)$ and $F_{\delta}(Q_i)$ respectively. Let $P=\langle p_1,p_2,\dots,p_n\rangle$ and $Q=\langle q_1,q_2,\dots,q_n\rangle$. Then $F_{\delta}(P_i)\sim \bern(1-e^{-\delta p_i})$ and $F_{\delta}(Q_i)\sim \bern(1-e^{-\delta q_i})$. 
\begin{align*}
\dchisqr(F_{\delta}(P),F_{\delta}(Q))&=\prod_i (1+\dchisqr(F_{\delta}(P_i),F_{\delta}(Q_i)))-1
&&\tag{From \cref{lem-chisq-mult}}\\
& \le \prod_i \exp(\dchisqr(F_{\delta}(P_i),F_{\delta}(Q_i))) -1 &&\tag{Since $e^x\ge (1+x)$ for $x\ge 0$}\\
&= \exp(\sum_i \dchisqr(F_{\delta}(P_i),F_{\delta}(Q_i)))-1\\
&= \exp\left(\sum_i (e^{-\delta p_i}-e^{-\delta q_i})^2\left({1\over e^{-\delta q_i}}+{1\over 1-e^{-\delta q_i}}\right)\right) -1
&& \tag{Since $F_{\delta}(P^{yes}_i)\sim \bern(1-e^{-\delta p_i})$ and $F_{\delta}(Q_i)\sim \bern(1-e^{-\delta q_i})$}\\
&= \exp(\sum_i (e^{-\delta p_i}-e^{-\delta q_i})^2/e^{-\delta q_i}(1-e^{-\delta q_i})) -1\\
&= \exp(\sum_i (e^{\delta (q_i-p_i)}-1)^2/(e^{\delta q_i}-1)) -1\\
&= \exp(\sum_i (e^{\delta (q_i-p_i)}-1)^2/(e^{\delta q_i}-1)) -1\\
&\le \exp(\sum_i (2\delta (p_i-q_i))^2/\delta q_i)) -1
&&\tag{Since $(e^x-1)\ge x$ and $(|e^{x}-1|\le 2|x|$ for $0<|x|<1$}\\
&= \exp(4\delta \chi^2(P,Q))-1.\\
\end{align*}
\end{proof}

\unstrKLonesample*
\begin{proof}
The proof of this Theorem appears in~\cite{Daskalakis:2018:DDS:3174304.3175479} (in Theorem 6.2 of this version), except the fact $||P^{yes}||_2^2=O(\log^2 n/n)$ is not explicitly claimed. We prove this claim in the following, by observing from the original construction given in the paper by~\cite{ValiantV10}.

The hard distribution $P^{yes}$ is the distribution $p^{-}_{\log k,\phi}$
as defined in Definition 12 of~\cite{ValiantV10}. We use the following facts about this distribution $p^{-}_{\log k,\phi}$, given in Fact 11, Definition 12 and (in the end of the second paragraph in the proof of) Lemma 13 in~\cite{ValiantV10}:
\begin{itemize}
\item $\phi$ is a small enough constant
\item The support size $n$ and the parameter $k$ are related as $n=32k\log k/\phi$
\item The `un-normalized' mass at each point is $x/32k$, where $j=\log k$ and $x\le 4j$
\item The `normalizing constant' $c_2$ (which makes the probability values sum up to 1) is at most $\phi/j$ where $j=\log k$
\end{itemize}
From these facts we conclude each probability mass is $c_2\cdot x/32k\le \phi/8k$, where $n=32k\log k/\phi$ for some constant $\phi$. Hence, $||P^{yes}||_2^2 \le \phi^2/64k^2\cdot 32k\log k/\phi=\phi\log k/2k=O(\log^2 n/n)$.
\end{proof}

\KLFdelta*
\begin{proof}
We use the following fact about the $\mathrm{KL}$-distance between two product distributions.
\begin{factRe}\label{lem-kl-additive}
For two distributions $P=\prod_{i=1}^n P_i$ and $Q=\prod_{i=1}^nQ_i$
over the same discrete sample space, it holds that
$\dkl(P,Q)= \sum_{i=1}^n \dkl(P_i,Q_i)$.
\end{factRe}
From \cref{fact-fdeltap}, both $F_{\delta}(P)$ and $F_{\delta}(Q)$ are product distributions, the 
distribution of the $i$-th component being $F_{\delta}(P_i)$ and $F_{\delta}(Q_i)$ respectively. Let $P=\langle p_1,p_2,\dots,p_n\rangle$ and $Q=\langle q_1,q_2,\dots,q_n\rangle$. Then $F_{\delta}(P_i)\sim \bern(1-e^{-\delta p_i})$ and $F_{\delta}(Q_i)\sim \bern(1-e^{-\delta q_i})$. 
\begin{align*}
\dkl(F_{\delta}(P),F_{\delta}(Q))&=\sum_i \dkl(F_{\delta}(P_i),F_{\delta}(Q_i))\\
&=\sum_i \left[(1-e^{-\delta p_i})\ln \left({1-e^{-\delta p_i}\over 1-e^{-\delta q_i}}\right)+e^{-\delta p_i}\ln {e^{-\delta p_i} \over e^{-\delta q_i}}\right]\\
&=\sum_i \ln \left({1-e^{-\delta p_i}\over 1-e^{-\delta q_i}}\right)+\sum_i e^{-\delta p_i} \ln {
e^{-\delta p_i} (1-e^{-\delta q_i}) \over
e^{-\delta q_i} (1-e^{-\delta p_i})
}\\
&=\sum_i \ln { e^{\delta q_i}(e^{\delta p_i}-1)\over e^{\delta p_i}(e^{\delta q_i}-1)}+
\sum_i e^{-\delta p_i} \ln \left({ e^{\delta q_i}-1\over e^{\delta p_i}-1}\right)\\
&=\sum_i \ln {e^{\delta q_i} \over e^{\delta p_i}} + \sum_i \ln \left({ e^{\delta p_i}-1\over e^{\delta q_i}-1}\right)+\sum_i e^{-\delta p_i} \ln \left({ e^{\delta q_i}-1\over e^{\delta p_i}-1}\right)\\
&=\sum_i (q_i-p_i) + \sum_i (1-e^{-\delta p_i})\ln \left({ e^{\delta p_i}-1\over e^{\delta q_i}-1}\right)\\
&=\sum_i (1-e^{-\delta p_i})\ln \left({ e^{\delta p_i}-1\over e^{\delta q_i}-1}\right) &&\tag{Since $\sum_i p_i=\sum_i q_i = 1$}\\
&\le \sum_i \delta p_i\ln \left({ \delta p_i (1+\delta p_i)\over \delta q_i}\right) &&\tag{Since $1-e^{-x}\le x$, and $x \le e^x-1 \le x(1+x)$ for $x<1$}\\
&= \delta\sum_i p_i \ln {p_i\over q_i}+ \delta \sum_i p_i \ln (1+\delta p_i) \\
&\le \delta \dkl(P,Q)+ \delta^2 \sum_i p_i^2. &&\tag{Using $\ln(1+x)\le x$}
\end{align*}
\end{proof}

==> dtvtol2sam.tex <==
\subsection{$\dtv$-tolerant 2-sample tester}
\citet*{bhattacharyya2020efficient} have given a $\dtv$-versus-$\dtv$ tester for Bayesian networks of degree at most $d$ with $O(|\Sigma|n\log n/\epsilon^2)$ samples.
Next, we give an algorithm for testing $\dtv(P,Q) \le \epsilon$ versus $\dtv(P,Q) > 3\epsilon$, for two product distributions $P$ and $Q$ over $\Sigma^n$. We use a testing-by-learning approach similar to \cref{sec:heltol-2S}.

As in \cref{sec:heltol-2S}, we first obtain a $\hat{P}$ such that $\dtv(P,\hat{P}) \le \sqrt{2}\dhel(P,\hat{P}) \le \epsilon/3$, and similarly a $\hat{Q}$, using $m=O(n(|\Sigma|+\log {n})/\epsilon^2)$ samples and $O(mn)$ time, with $1-1/n$ probability. Conditioned on this, it suffices to estimate $\dtv(\hat{P},\hat{Q})$ up to an additive $\epsilon/3$ error with $1-1/n$ probability. We use the following result.

\begin{theoremRe}\citep*{bhattacharyya2020efficient}
Given two fixed product distributions $R$ and $S$ over $\Sigma^n$, $\dtv(R,S)$ can be estimated up to additive $\epsilon$ error with $1-\delta$ probability in $O(n\log {1\over \delta}/\epsilon^2)$ time. 
\end{theoremRe}

